Learning Primal Heuristics for Mixed Integer Programs

This paper proposes a novel primal heuristic for Mixed Integer Programs, by employing machine learning techniques. Mixed Integer Programming is a general technique for formulating combinatorial optimization problems. Inside a solver, primal heuristics play a critical role in finding good feasible solutions that enable one to tighten the duality gap from the outset of the Branch-and-Bound algorithm (B&B), greatly improving its performance by pruning the B&B tree aggressively. In this paper, we investigate whether effective primal heuristics can be automatically learned via machine learning. We propose a new method to represent an optimization problem as a graph, and train a Graph Convolutional Network on solved problem instances with known optimal solutions. This in turn can predict the values of decision variables in the optimal solution for an unseen problem instance of a similar type. The prediction of variable solutions is then leveraged by a novel configuration of the B&B method, Probabilistic Branching with guided Depth-first Search (PB-DFS) approach, aiming to find (near-)optimal solutions quickly. The experimental results show that this new heuristic can find better primal solutions at a much earlier stage of the solving process, compared to other state-of-the-art primal heuristics.

==> 2-relatedwork.tex <==
\section{Related work}
\label{sec:related}

There are a number of studies using machine learning to improve the performance of MIP solvers in finding good primal solutions. Ding et al. \cite{ding2019optimal} uses predicted solutions by a GCN variant with a tripartite graph representation of an MIP instance to generate local branching cuts to reduce the size of a problem. Sun et al. \cite{sun2019using} uses support vector machine (SVM) with general statistical measures as variable's features to reduce the search space of the Maximum Weighted Clique problem. \cite{he2014learning} learns separate SVM models to decide whether to plunge or discard a certain node, aiming to devote more of the computational budget on nodes that are likely to contain an optimal solution. \cite{khalil2017learning} learns a SVM model to decide what heuristics to run at a certain node. Other work develops heuristics outside the B\&B framework, for instance, \cite{khalil2017learning} uses GCN variant trained via reinforcement learning to greedily construct solutions for a problem; \cite{li2018combinatorial} applies GCN to predict the solutions of variables in an optimal solution, and the feasibility of which is resolved by a greedy algorithmic approach. For a comprehensive overview, we refer readers to the survey paper \cite{bengio2018machine}.

% whose feasible set 


